Source Coding with Mismatched Distortion Measures

We consider the problem of lossy source coding with a mismatched distortion measure. That is, we investigate what distortion guarantees can be made with respect to distortion measure $\tilde{\rho}$, for a source code designed such that it achieves distortion less than $D$ with respect to distortion measure $\rho$. We find a single-letter characterization of this mismatch distortion and study properties of this quantity. These results give insight into the robustness of lossy source coding with respect to modeling errors in the distortion measure. They also provide guidelines on how to choose a good tractable approximation of an intractable distortion measure.

==> figs/gauss.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup%
  \makeatletter%
  \newcommand{\GNUPLOTspecial}{%
    \@sanitize\catcode`\%=14\relax\special}%
  \setlength{\unitlength}{0.1bp}%
\begin{picture}(3600,2160)(0,0)%
{\GNUPLOTspecial{"
%!PS-Adobe-2.0 EPSF-2.0
%%Title: gauss.tex
%%Creator: gnuplot 4.0 patchlevel 0
%%CreationDate: Wed Dec 19 22:52:17 2007
%%DocumentFonts: 
%%BoundingBox: 0 0 360 216
%%Orientation: Landscape
%%EndComments
/gnudict 256 dict def
gnudict begin
/Color false def
/Solid false def
/gnulinewidth 5.000 def
/userlinewidth gnulinewidth def
/vshift -33 def
/dl {10.0 mul} def
/hpt_ 31.5 def
/vpt_ 31.5 def
/hpt hpt_ def
/vpt vpt_ def
/Rounded false def
/M {moveto} bind def
/L {lineto} bind def
/R {rmoveto} bind def
/V {rlineto} bind def
/N {newpath moveto} bind def
/C {setrgbcolor} bind def
/f {rlineto fill} bind def
/vpt2 vpt 2 mul def
/hpt2 hpt 2 mul def
/Lshow { currentpoint stroke M
  0 vshift R show } def
/Rshow { currentpoint stroke M
  dup stringwidth pop neg vshift R show } def
/Cshow { currentpoint stroke M
  dup stringwidth pop -2 div vshift R show } def
/UP { dup vpt_ mul /vpt exch def hpt_ mul /hpt exch def
  /hpt2 hpt 2 mul def /vpt2 vpt 2 mul def } def
/DL { Color {setrgbcolor Solid {pop []} if 0 setdash }
 {pop pop pop 0 setgray Solid {pop []} if 0 setdash} ifelse } def
/BL { stroke userlinewidth 2 mul setlinewidth
      Rounded { 1 setlinejoin 1 setlinecap } if } def
/AL { stroke userlinewidth 2 div setlinewidth
      Rounded { 1 setlinejoin 1 setlinecap } if } def
/UL { dup gnulinewidth mul /userlinewidth exch def
      dup 1 lt {pop 1} if 10 mul /udl exch def } def
/PL { stroke userlinewidth setlinewidth
      Rounded { 1 setlinejoin 1 setlinecap } if } def
/LTw { PL [] 1 setgray } def
/LTb { BL [] 0 0 0 DL } def
/LTa { AL [1 udl mul 2 udl mul] 0 setdash 0 0 0 setrgbcolor } def
/LT0 { PL [] 1 0 0 DL } def
/LT1 { PL [4 dl 2 dl] 0 1 0 DL } def
/LT2 { PL [2 dl 3 dl] 0 0 1 DL } def
/LT3 { PL [1 dl 1.5 dl] 1 0 1 DL } def
/LT4 { PL [5 dl 2 dl 1 dl 2 dl] 0 1 1 DL } def
/LT5 { PL [4 dl 3 dl 1 dl 3 dl] 1 1 0 DL } def
/LT6 { PL [2 dl 2 dl 2 dl 4 dl] 0 0 0 DL } def
/LT7 { PL [2 dl 2 dl 2 dl 2 dl 2 dl 4 dl] 1 0.3 0 DL } def
/LT8 { PL [2 dl 2 dl 2 dl 2 dl 2 dl 2 dl 2 dl 4 dl] 0.5 0.5 0.5 DL } def
/Pnt { stroke [] 0 setdash
   gsave 1 setlinecap M 0 0 V stroke grestore } def
/Dia { stroke [] 0 setdash 2 copy vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke
  Pnt } def
/Pls { stroke [] 0 setdash vpt sub M 0 vpt2 V
  currentpoint stroke M
  hpt neg vpt neg R hpt2 0 V stroke
  } def
/Box { stroke [] 0 setdash 2 copy exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke
  Pnt } def
/Crs { stroke [] 0 setdash exch hpt sub exch vpt add M
  hpt2 vpt2 neg V currentpoint stroke M
  hpt2 neg 0 R hpt2 vpt2 V stroke } def
/TriU { stroke [] 0 setdash 2 copy vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke
  Pnt  } def
/Star { 2 copy Pls Crs } def
/BoxF { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V  hpt2 0 V  0 vpt2 V
  hpt2 neg 0 V  closepath fill } def
/TriUF { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath fill } def
/TriD { stroke [] 0 setdash 2 copy vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke
  Pnt  } def
/TriDF { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath fill} def
/DiaF { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath fill } def
/Pent { stroke [] 0 setdash 2 copy gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore Pnt } def
/PentF { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath fill grestore } def
/Circle { stroke [] 0 setdash 2 copy
  hpt 0 360 arc stroke Pnt } def
/CircleF { stroke [] 0 setdash hpt 0 360 arc fill } def
/C0 { BL [] 0 setdash 2 copy moveto vpt 90 450  arc } bind def
/C1 { BL [] 0 setdash 2 copy        moveto
       2 copy  vpt 0 90 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C2 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 90 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C3 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C4 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 180 270 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C5 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 90 arc
       2 copy moveto
       2 copy  vpt 180 270 arc closepath fill
               vpt 0 360 arc } bind def
/C6 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 90 270 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C7 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 0 270 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C8 { BL [] 0 setdash 2 copy moveto
      2 copy vpt 270 360 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C9 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 270 450 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C10 { BL [] 0 setdash 2 copy 2 copy moveto vpt 270 360 arc closepath fill
       2 copy moveto
       2 copy vpt 90 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C11 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 180 arc closepath fill
       2 copy moveto
       2 copy  vpt 270 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C12 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 180 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C13 { BL [] 0 setdash  2 copy moveto
       2 copy  vpt 0 90 arc closepath fill
       2 copy moveto
       2 copy  vpt 180 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C14 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 90 360 arc closepath fill
               vpt 0 360 arc } bind def
/C15 { BL [] 0 setdash 2 copy vpt 0 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/Rec   { newpath 4 2 roll moveto 1 index 0 rlineto 0 exch rlineto
       neg 0 rlineto closepath } bind def
/Square { dup Rec } bind def
/Bsquare { vpt sub exch vpt sub exch vpt2 Square } bind def
/S0 { BL [] 0 setdash 2 copy moveto 0 vpt rlineto BL Bsquare } bind def
/S1 { BL [] 0 setdash 2 copy vpt Square fill Bsquare } bind def
/S2 { BL [] 0 setdash 2 copy exch vpt sub exch vpt Square fill Bsquare } bind def
/S3 { BL [] 0 setdash 2 copy exch vpt sub exch vpt2 vpt Rec fill Bsquare } bind def
/S4 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt Square fill Bsquare } bind def
/S5 { BL [] 0 setdash 2 copy 2 copy vpt Square fill
       exch vpt sub exch vpt sub vpt Square fill Bsquare } bind def
/S6 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill Bsquare } bind def
/S7 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill
       2 copy vpt Square fill
       Bsquare } bind def
/S8 { BL [] 0 setdash 2 copy vpt sub vpt Square fill Bsquare } bind def
/S9 { BL [] 0 setdash 2 copy vpt sub vpt vpt2 Rec fill Bsquare } bind def
/S10 { BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt Square fill
       Bsquare } bind def
/S11 { BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt2 vpt Rec fill
       Bsquare } bind def
/S12 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill Bsquare } bind def
/S13 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
       2 copy vpt Square fill Bsquare } bind def
/S14 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
       2 copy exch vpt sub exch vpt Square fill Bsquare } bind def
/S15 { BL [] 0 setdash 2 copy Bsquare fill Bsquare } bind def
/D0 { gsave translate 45 rotate 0 0 S0 stroke grestore } bind def
/D1 { gsave translate 45 rotate 0 0 S1 stroke grestore } bind def
/D2 { gsave translate 45 rotate 0 0 S2 stroke grestore } bind def
/D3 { gsave translate 45 rotate 0 0 S3 stroke grestore } bind def
/D4 { gsave translate 45 rotate 0 0 S4 stroke grestore } bind def
/D5 { gsave translate 45 rotate 0 0 S5 stroke grestore } bind def
/D6 { gsave translate 45 rotate 0 0 S6 stroke grestore } bind def
/D7 { gsave translate 45 rotate 0 0 S7 stroke grestore } bind def
/D8 { gsave translate 45 rotate 0 0 S8 stroke grestore } bind def
/D9 { gsave translate 45 rotate 0 0 S9 stroke grestore } bind def
/D10 { gsave translate 45 rotate 0 0 S10 stroke grestore } bind def
/D11 { gsave translate 45 rotate 0 0 S11 stroke grestore } bind def
/D12 { gsave translate 45 rotate 0 0 S12 stroke grestore } bind def
/D13 { gsave translate 45 rotate 0 0 S13 stroke grestore } bind def
/D14 { gsave translate 45 rotate 0 0 S14 stroke grestore } bind def
/D15 { gsave translate 45 rotate 0 0 S15 stroke grestore } bind def
/DiaE { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke } def
/BoxE { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke } def
/TriUE { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke } def
/TriDE { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke } def
/PentE { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore } def
/CircE { stroke [] 0 setdash 
  hpt 0 360 arc stroke } def
/Opaque { gsave closepath 1 setgray fill grestore 0 setgray closepath } def
/DiaW { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V Opaque stroke } def
/BoxW { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V Opaque stroke } def
/TriUW { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V Opaque stroke } def
/TriDW { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V Opaque stroke } def
/PentW { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  Opaque stroke grestore } def
/CircW { stroke [] 0 setdash 
  hpt 0 360 arc Opaque stroke } def
/BoxFill { gsave Rec 1 setgray fill grestore } def
/BoxColFill {
  gsave Rec
  /Fillden exch def
  currentrgbcolor
  /ColB exch def /ColG exch def /ColR exch def
  /ColR ColR Fillden mul Fillden sub 1 add def
  /ColG ColG Fillden mul Fillden sub 1 add def
  /ColB ColB Fillden mul Fillden sub 1 add def
  ColR ColG ColB setrgbcolor
  fill grestore } def
%
% PostScript Level 1 Pattern Fill routine
% Usage: x y w h s a XX PatternFill
%	x,y = lower left corner of box to be filled
%	w,h = width and height of box
%	  a = angle in degrees between lines and x-axis
%	 XX = 0/1 for no/yes cross-hatch
%
/PatternFill { gsave /PFa [ 9 2 roll ] def
    PFa 0 get PFa 2 get 2 div add PFa 1 get PFa 3 get 2 div add translate
    PFa 2 get -2 div PFa 3 get -2 div PFa 2 get PFa 3 get Rec
    gsave 1 setgray fill grestore clip
    currentlinewidth 0.5 mul setlinewidth
    /PFs PFa 2 get dup mul PFa 3 get dup mul add sqrt def
    0 0 M PFa 5 get rotate PFs -2 div dup translate
	0 1 PFs PFa 4 get div 1 add floor cvi
	{ PFa 4 get mul 0 M 0 PFs V } for
    0 PFa 6 get ne {
	0 1 PFs PFa 4 get div 1 add floor cvi
	{ PFa 4 get mul 0 2 1 roll M PFs 0 V } for
    } if
    stroke grestore } def
%
/Symbol-Oblique /Symbol findfont [1 0 .167 1 0 0] makefont
dup length dict begin {1 index /FID eq {pop pop} {def} ifelse} forall
currentdict end definefont pop
end
%%EndProlog
gnudict begin
gsave
0 0 translate
0.100 0.100 scale
0 setgray
newpath
1.000 UL
LTb
350 300 M
63 0 V
3037 0 R
-63 0 V
1.000 UL
LTb
350 652 M
63 0 V
3037 0 R
-63 0 V
1.000 UL
LTb
350 1004 M
63 0 V
3037 0 R
-63 0 V
1.000 UL
LTb
350 1356 M
63 0 V
3037 0 R
-63 0 V
1.000 UL
LTb
350 1708 M
63 0 V
3037 0 R
-63 0 V
1.000 UL
LTb
350 2060 M
63 0 V
3037 0 R
-63 0 V
1.000 UL
LTb
350 300 M
0 63 V
0 1697 R
0 -63 V
1.000 UL
LTb
1125 300 M
0 63 V
0 1697 R
0 -63 V
1.000 UL
LTb
1900 300 M
0 63 V
0 1697 R
0 -63 V
1.000 UL
LTb
2675 300 M
0 63 V
0 1697 R
0 -63 V
1.000 UL
LTb
3450 300 M
0 63 V
0 1697 R
0 -63 V
1.000 UL
LTb
1.000 UL
LTb
350 300 M
3100 0 V
0 1760 V
-3100 0 V
350 300 L
LTb
1.000 UP
1.000 UL
LT0
LTb
LT0
3063 652 M
263 0 V
350 1400 M
10 76 V
11 31 V
10 24 V
10 20 V
11 17 V
10 15 V
11 14 V
10 13 V
10 12 V
11 12 V
10 10 V
10 10 V
11 10 V
10 9 V
11 8 V
10 9 V
10 8 V
11 7 V
10 8 V
10 7 V
11 7 V
10 6 V
10 7 V
11 6 V
10 6 V
11 6 V
10 5 V
10 6 V
11 5 V
10 5 V
10 6 V
11 4 V
10 5 V
11 5 V
10 5 V
10 4 V
11 4 V
10 5 V
10 4 V
11 4 V
10 4 V
10 4 V
11 4 V
10 3 V
11 4 V
10 3 V
10 4 V
11 3 V
10 4 V
10 3 V
11 3 V
10 3 V
10 3 V
11 3 V
10 3 V
11 3 V
10 3 V
10 3 V
11 3 V
10 2 V
10 3 V
11 3 V
10 2 V
11 3 V
10 2 V
10 2 V
11 3 V
10 2 V
10 2 V
11 3 V
10 2 V
10 2 V
11 2 V
10 2 V
11 2 V
10 2 V
10 2 V
11 2 V
10 2 V
10 2 V
11 2 V
10 2 V
11 1 V
10 2 V
10 2 V
11 2 V
10 1 V
10 2 V
11 2 V
10 1 V
10 2 V
11 1 V
10 2 V
11 1 V
10 2 V
10 1 V
11 2 V
10 1 V
10 1 V
11 2 V
10 1 V
11 1 V
stroke
1408 1969 M
10 2 V
10 1 V
11 1 V
10 2 V
10 1 V
11 1 V
10 1 V
10 1 V
11 1 V
10 2 V
11 1 V
10 1 V
10 1 V
11 1 V
10 1 V
10 1 V
11 1 V
10 1 V
11 1 V
10 1 V
10 1 V
11 1 V
10 1 V
10 1 V
11 1 V
10 0 V
10 1 V
11 1 V
10 1 V
11 1 V
10 1 V
10 1 V
11 0 V
10 1 V
10 1 V
11 1 V
10 0 V
11 1 V
10 1 V
10 1 V
11 0 V
10 1 V
10 1 V
11 0 V
10 1 V
10 1 V
11 0 V
10 1 V
11 1 V
10 0 V
10 1 V
11 1 V
10 0 V
10 1 V
11 0 V
10 1 V
10 0 V
11 1 V
10 1 V
11 0 V
10 1 V
10 0 V
11 1 V
10 0 V
10 1 V
11 0 V
10 1 V
11 0 V
10 1 V
10 0 V
11 1 V
10 0 V
10 0 V
11 1 V
10 0 V
10 1 V
11 0 V
10 1 V
11 0 V
10 0 V
10 1 V
11 0 V
10 1 V
10 0 V
11 0 V
10 1 V
11 0 V
10 0 V
10 1 V
11 0 V
10 1 V
10 0 V
11 0 V
10 1 V
10 0 V
11 0 V
10 1 V
11 0 V
10 0 V
10 0 V
11 1 V
10 0 V
10 0 V
11 1 V
stroke
2486 2039 M
10 0 V
11 0 V
10 1 V
10 0 V
11 0 V
10 0 V
10 1 V
11 0 V
10 0 V
10 0 V
11 1 V
10 0 V
11 0 V
10 0 V
10 1 V
11 0 V
10 0 V
10 0 V
11 1 V
10 0 V
11 0 V
10 0 V
10 0 V
11 1 V
10 0 V
10 0 V
11 0 V
10 0 V
10 1 V
11 0 V
10 0 V
11 0 V
10 0 V
10 1 V
11 0 V
10 0 V
10 0 V
11 0 V
10 0 V
11 1 V
10 0 V
10 0 V
11 0 V
10 0 V
10 0 V
11 1 V
10 0 V
10 0 V
11 0 V
10 0 V
11 0 V
10 0 V
10 1 V
11 0 V
10 0 V
10 0 V
11 0 V
10 0 V
10 0 V
11 1 V
10 0 V
11 0 V
10 0 V
10 0 V
11 0 V
10 0 V
10 0 V
11 1 V
10 0 V
11 0 V
10 0 V
10 0 V
11 0 V
10 0 V
10 0 V
11 0 V
10 0 V
10 1 V
11 0 V
10 0 V
11 0 V
10 0 V
10 0 V
11 0 V
10 0 V
10 0 V
11 0 V
10 1 V
11 0 V
10 0 V
10 0 V
11 0 V
10 0 V
1.000 UL
LTb
350 300 M
3100 0 V
0 1760 V
-3100 0 V
350 300 L
1.000 UP
stroke
grestore
end
showpage
}}%
\put(3013,652){\makebox(0,0)[r]{$\msf{D_{\rho,\tilde{\rho}}}(\msf{R_{\rho}}(D_{\rho})+r,D_{\rho})/\msf{D_{\rho,\tilde{\rho}}}(\infty,D_{\rho})$}}%
\put(1900,50){\makebox(0,0){$r$}}%
\put(3450,200){\makebox(0,0){ 2}}%
\put(2675,200){\makebox(0,0){ 1.5}}%
\put(1900,200){\makebox(0,0){ 1}}%
\put(1125,200){\makebox(0,0){ 0.5}}%
\put(350,200){\makebox(0,0){ 0}}%
\put(300,2060){\makebox(0,0)[r]{ 1}}%
\put(300,1708){\makebox(0,0)[r]{ 0.8}}%
\put(300,1356){\makebox(0,0)[r]{ 0.6}}%
\put(300,1004){\makebox(0,0)[r]{ 0.4}}%
\put(300,652){\makebox(0,0)[r]{ 0.2}}%
\put(300,300){\makebox(0,0)[r]{ 0}}%
\end{picture}%
\endgroup
\endinput


==> figs/mismatch.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup%
  \makeatletter%
  \newcommand{\GNUPLOTspecial}{%
    \@sanitize\catcode`\%=14\relax\special}%
  \setlength{\unitlength}{0.1bp}%
\begin{picture}(3600,2160)(0,0)%
{\GNUPLOTspecial{"
%!PS-Adobe-2.0 EPSF-2.0
%%Title: mismatch.tex
%%Creator: gnuplot 4.0 patchlevel 0
%%CreationDate: Tue Mar  6 21:01:49 2007
%%DocumentFonts: 
%%BoundingBox: 0 0 360 216
%%Orientation: Landscape
%%EndComments
/gnudict 256 dict def
gnudict begin
/Color false def
/Solid false def
/gnulinewidth 5.000 def
/userlinewidth gnulinewidth def
/vshift -33 def
/dl {10.0 mul} def
/hpt_ 31.5 def
/vpt_ 31.5 def
/hpt hpt_ def
/vpt vpt_ def
/Rounded false def
/M {moveto} bind def
/L {lineto} bind def
/R {rmoveto} bind def
/V {rlineto} bind def
/N {newpath moveto} bind def
/C {setrgbcolor} bind def
/f {rlineto fill} bind def
/vpt2 vpt 2 mul def
/hpt2 hpt 2 mul def
/Lshow { currentpoint stroke M
  0 vshift R show } def
/Rshow { currentpoint stroke M
  dup stringwidth pop neg vshift R show } def
/Cshow { currentpoint stroke M
  dup stringwidth pop -2 div vshift R show } def
/UP { dup vpt_ mul /vpt exch def hpt_ mul /hpt exch def
  /hpt2 hpt 2 mul def /vpt2 vpt 2 mul def } def
/DL { Color {setrgbcolor Solid {pop []} if 0 setdash }
 {pop pop pop 0 setgray Solid {pop []} if 0 setdash} ifelse } def
/BL { stroke userlinewidth 2 mul setlinewidth
      Rounded { 1 setlinejoin 1 setlinecap } if } def
/AL { stroke userlinewidth 2 div setlinewidth
      Rounded { 1 setlinejoin 1 setlinecap } if } def
/UL { dup gnulinewidth mul /userlinewidth exch def
      dup 1 lt {pop 1} if 10 mul /udl exch def } def
/PL { stroke userlinewidth setlinewidth
      Rounded { 1 setlinejoin 1 setlinecap } if } def
/LTw { PL [] 1 setgray } def
/LTb { BL [] 0 0 0 DL } def
/LTa { AL [1 udl mul 2 udl mul] 0 setdash 0 0 0 setrgbcolor } def
/LT0 { PL [] 1 0 0 DL } def
/LT1 { PL [4 dl 2 dl] 0 1 0 DL } def
/LT2 { PL [2 dl 3 dl] 0 0 1 DL } def
/LT3 { PL [1 dl 1.5 dl] 1 0 1 DL } def
/LT4 { PL [5 dl 2 dl 1 dl 2 dl] 0 1 1 DL } def
/LT5 { PL [4 dl 3 dl 1 dl 3 dl] 1 1 0 DL } def
/LT6 { PL [2 dl 2 dl 2 dl 4 dl] 0 0 0 DL } def
/LT7 { PL [2 dl 2 dl 2 dl 2 dl 2 dl 4 dl] 1 0.3 0 DL } def
/LT8 { PL [2 dl 2 dl 2 dl 2 dl 2 dl 2 dl 2 dl 4 dl] 0.5 0.5 0.5 DL } def
/Pnt { stroke [] 0 setdash
   gsave 1 setlinecap M 0 0 V stroke grestore } def
/Dia { stroke [] 0 setdash 2 copy vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke
  Pnt } def
/Pls { stroke [] 0 setdash vpt sub M 0 vpt2 V
  currentpoint stroke M
  hpt neg vpt neg R hpt2 0 V stroke
  } def
/Box { stroke [] 0 setdash 2 copy exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke
  Pnt } def
/Crs { stroke [] 0 setdash exch hpt sub exch vpt add M
  hpt2 vpt2 neg V currentpoint stroke M
  hpt2 neg 0 R hpt2 vpt2 V stroke } def
/TriU { stroke [] 0 setdash 2 copy vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke
  Pnt  } def
/Star { 2 copy Pls Crs } def
/BoxF { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V  hpt2 0 V  0 vpt2 V
  hpt2 neg 0 V  closepath fill } def
/TriUF { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath fill } def
/TriD { stroke [] 0 setdash 2 copy vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke
  Pnt  } def
/TriDF { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath fill} def
/DiaF { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath fill } def
/Pent { stroke [] 0 setdash 2 copy gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore Pnt } def
/PentF { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath fill grestore } def
/Circle { stroke [] 0 setdash 2 copy
  hpt 0 360 arc stroke Pnt } def
/CircleF { stroke [] 0 setdash hpt 0 360 arc fill } def
/C0 { BL [] 0 setdash 2 copy moveto vpt 90 450  arc } bind def
/C1 { BL [] 0 setdash 2 copy        moveto
       2 copy  vpt 0 90 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C2 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 90 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C3 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C4 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 180 270 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C5 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 90 arc
       2 copy moveto
       2 copy  vpt 180 270 arc closepath fill
               vpt 0 360 arc } bind def
/C6 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 90 270 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C7 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 0 270 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C8 { BL [] 0 setdash 2 copy moveto
      2 copy vpt 270 360 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C9 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 270 450 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C10 { BL [] 0 setdash 2 copy 2 copy moveto vpt 270 360 arc closepath fill
       2 copy moveto
       2 copy vpt 90 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C11 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 180 arc closepath fill
       2 copy moveto
       2 copy  vpt 270 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C12 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 180 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C13 { BL [] 0 setdash  2 copy moveto
       2 copy  vpt 0 90 arc closepath fill
       2 copy moveto
       2 copy  vpt 180 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C14 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 90 360 arc closepath fill
               vpt 0 360 arc } bind def
/C15 { BL [] 0 setdash 2 copy vpt 0 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/Rec   { newpath 4 2 roll moveto 1 index 0 rlineto 0 exch rlineto
       neg 0 rlineto closepath } bind def
/Square { dup Rec } bind def
/Bsquare { vpt sub exch vpt sub exch vpt2 Square } bind def
/S0 { BL [] 0 setdash 2 copy moveto 0 vpt rlineto BL Bsquare } bind def
/S1 { BL [] 0 setdash 2 copy vpt Square fill Bsquare } bind def
/S2 { BL [] 0 setdash 2 copy exch vpt sub exch vpt Square fill Bsquare } bind def
/S3 { BL [] 0 setdash 2 copy exch vpt sub exch vpt2 vpt Rec fill Bsquare } bind def
/S4 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt Square fill Bsquare } bind def
/S5 { BL [] 0 setdash 2 copy 2 copy vpt Square fill
       exch vpt sub exch vpt sub vpt Square fill Bsquare } bind def
/S6 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill Bsquare } bind def
/S7 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill
       2 copy vpt Square fill
       Bsquare } bind def
/S8 { BL [] 0 setdash 2 copy vpt sub vpt Square fill Bsquare } bind def
/S9 { BL [] 0 setdash 2 copy vpt sub vpt vpt2 Rec fill Bsquare } bind def
/S10 { BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt Square fill
       Bsquare } bind def
/S11 { BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt2 vpt Rec fill
       Bsquare } bind def
/S12 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill Bsquare } bind def
/S13 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
       2 copy vpt Square fill Bsquare } bind def
/S14 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
       2 copy exch vpt sub exch vpt Square fill Bsquare } bind def
/S15 { BL [] 0 setdash 2 copy Bsquare fill Bsquare } bind def
/D0 { gsave translate 45 rotate 0 0 S0 stroke grestore } bind def
/D1 { gsave translate 45 rotate 0 0 S1 stroke grestore } bind def
/D2 { gsave translate 45 rotate 0 0 S2 stroke grestore } bind def
/D3 { gsave translate 45 rotate 0 0 S3 stroke grestore } bind def
/D4 { gsave translate 45 rotate 0 0 S4 stroke grestore } bind def
/D5 { gsave translate 45 rotate 0 0 S5 stroke grestore } bind def
/D6 { gsave translate 45 rotate 0 0 S6 stroke grestore } bind def
/D7 { gsave translate 45 rotate 0 0 S7 stroke grestore } bind def
/D8 { gsave translate 45 rotate 0 0 S8 stroke grestore } bind def
/D9 { gsave translate 45 rotate 0 0 S9 stroke grestore } bind def
/D10 { gsave translate 45 rotate 0 0 S10 stroke grestore } bind def
/D11 { gsave translate 45 rotate 0 0 S11 stroke grestore } bind def
/D12 { gsave translate 45 rotate 0 0 S12 stroke grestore } bind def
/D13 { gsave translate 45 rotate 0 0 S13 stroke grestore } bind def
/D14 { gsave translate 45 rotate 0 0 S14 stroke grestore } bind def
/D15 { gsave translate 45 rotate 0 0 S15 stroke grestore } bind def
/DiaE { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke } def
/BoxE { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke } def
/TriUE { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke } def
/TriDE { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke } def
/PentE { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore } def
/CircE { stroke [] 0 setdash 
  hpt 0 360 arc stroke } def
/Opaque { gsave closepath 1 setgray fill grestore 0 setgray closepath } def
/DiaW { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V Opaque stroke } def
/BoxW { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V Opaque stroke } def
/TriUW { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V Opaque stroke } def
/TriDW { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V Opaque stroke } def
/PentW { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  Opaque stroke grestore } def
/CircW { stroke [] 0 setdash 
  hpt 0 360 arc Opaque stroke } def
/BoxFill { gsave Rec 1 setgray fill grestore } def
/BoxColFill {
  gsave Rec
  /Fillden exch def
  currentrgbcolor
  /ColB exch def /ColG exch def /ColR exch def
  /ColR ColR Fillden mul Fillden sub 1 add def
  /ColG ColG Fillden mul Fillden sub 1 add def
  /ColB ColB Fillden mul Fillden sub 1 add def
  ColR ColG ColB setrgbcolor
  fill grestore } def
%
% PostScript Level 1 Pattern Fill routine
% Usage: x y w h s a XX PatternFill
%	x,y = lower left corner of box to be filled
%	w,h = width and height of box
%	  a = angle in degrees between lines and x-axis
%	 XX = 0/1 for no/yes cross-hatch
%
/PatternFill { gsave /PFa [ 9 2 roll ] def
    PFa 0 get PFa 2 get 2 div add PFa 1 get PFa 3 get 2 div add translate
    PFa 2 get -2 div PFa 3 get -2 div PFa 2 get PFa 3 get Rec
    gsave 1 setgray fill grestore clip
    currentlinewidth 0.5 mul setlinewidth
    /PFs PFa 2 get dup mul PFa 3 get dup mul add sqrt def
    0 0 M PFa 5 get rotate PFs -2 div dup translate
	0 1 PFs PFa 4 get div 1 add floor cvi
	{ PFa 4 get mul 0 M 0 PFs V } for
    0 PFa 6 get ne {
	0 1 PFs PFa 4 get div 1 add floor cvi
	{ PFa 4 get mul 0 2 1 roll M PFs 0 V } for
    } if
    stroke grestore } def
%
/Symbol-Oblique /Symbol findfont [1 0 .167 1 0 0] makefont
dup length dict begin {1 index /FID eq {pop pop} {def} ifelse} forall
currentdict end definefont pop
end
%%EndProlog
gnudict begin
gsave
0 0 translate
0.100 0.100 scale
0 setgray
newpath
1.000 UL
LTb
1.000 UP
1.000 UL
LT0
2951 802 M
2 -9 V
1.000 UL
LT0
2867 795 M
86 -2 V
1.000 UL
LT0
2947 812 M
4 -10 V
1.000 UL
LT0
2867 805 M
84 -3 V
1.000 UL
LT0
2941 824 M
6 -12 V
1.000 UL
LT0
2866 816 M
81 -4 V
1.000 UL
LT0
2935 838 M
6 -14 V
1.000 UL
LT0
2863 830 M
78 -6 V
1.000 UL
LT0
2926 854 M
9 -16 V
1.000 UL
LT0
2858 845 M
77 -7 V
1.000 UL
LT0
2867 805 M
0 -10 V
1.000 UL
LT0
2778 798 M
89 -3 V
1.000 UL
LT0
2916 872 M
10 -18 V
1.000 UL
LT0
2853 862 M
73 -8 V
1.000 UL
LT0
2866 816 M
1 -11 V
1.000 UL
LT0
2782 809 M
85 -4 V
1.000 UL
LT0
2863 830 M
3 -14 V
1.000 UL
LT0
2783 822 M
83 -6 V
1.000 UL
LT0
2905 892 M
11 -20 V
1.000 UL
LT0
2845 882 M
71 -10 V
1.000 UL
LT0
2858 845 M
5 -15 V
1.000 UL
LT0
2782 837 M
81 -7 V
1.000 UL
LT0
2891 915 M
14 -23 V
1.000 UL
LT0
2836 904 M
69 -12 V
1.000 UL
LT0
2853 862 M
5 -17 V
1.000 UL
LT0
2780 854 M
78 -9 V
1.000 UL
LT0
2875 940 M
16 -25 V
1.000 UL
LT0
2826 928 M
65 -13 V
1.000 UL
LT0
2845 882 M
8 -20 V
1.000 UL
LT0
2777 873 M
76 -11 V
1.000 UL
LT0
2782 809 M
-4 -11 V
1.000 UL
LT0
2687 804 M
91 -6 V
1.000 UL
LT0
2783 822 M
-1 -13 V
1.000 UL
LT0
2694 816 M
88 -7 V
1.000 UL
LT0
2836 904 M
9 -22 V
1.000 UL
LT0
2773 894 M
72 -12 V
1.000 UL
LT0
2856 968 M
19 -28 V
1.000 UL
LT0
2812 955 M
63 -15 V
1.000 UL
LT0
2782 837 M
1 -15 V
1.000 UL
LT0
2697 830 M
86 -8 V
1.000 UL
LT0
2826 928 M
10 -24 V
1.000 UL
LT0
2767 917 M
69 -13 V
1.000 UL
LT0
2780 854 M
2 -17 V
1.000 UL
LT0
2699 846 M
83 -9 V
1.000 UL
LT0
2834 1000 M
22 -32 V
1.000 UL
LT0
2796 984 M
60 -16 V
1.000 UL
LT0
2777 873 M
3 -19 V
1.000 UL
LT0
2700 864 M
80 -10 V
1.000 UL
LT0
2812 955 M
14 -27 V
1.000 UL
LT0
2759 943 M
67 -15 V
1.000 UL
LT0
2773 894 M
4 -21 V
1.000 UL
LT0
2700 885 M
77 -12 V
1.000 UL
LT0
2809 1035 M
25 -35 V
1.000 UL
LT0
2777 1017 M
57 -17 V
1.000 UL
LT0
2796 984 M
16 -29 V
1.000 UL
LT0
2748 971 M
64 -16 V
1.000 UL
LT0
2694 816 M
-7 -12 V
1.000 UL
LT0
2593 811 M
94 -7 V
1.000 UL
LT0
2767 917 M
6 -23 V
1.000 UL
LT0
2698 907 M
75 -13 V
1.000 UL
LT0
2697 830 M
-3 -14 V
1.000 UL
LT0
2603 824 M
91 -8 V
1.000 UL
LT0
2777 1017 M
19 -33 V
1.000 UL
LT0
2736 1002 M
60 -18 V
1.000 UL
LT0
2759 943 M
8 -26 V
1.000 UL
LT0
2695 932 M
72 -15 V
1.000 UL
LT0
2699 846 M
-2 -16 V
1.000 UL
LT0
2609 839 M
88 -9 V
1.000 UL
LT0
2780 1074 M
29 -39 V
1.000 UL
LT0
2755 1054 M
54 -19 V
1.000 UL
LT0
2700 864 M
-1 -18 V
1.000 UL
LT0
2614 857 M
85 -11 V
1.000 UL
LT0
2748 971 M
11 -28 V
1.000 UL
LT0
2690 960 M
69 -17 V
1.000 UL
LT0
2755 1054 M
22 -37 V
1.000 UL
LT0
2719 1037 M
58 -20 V
1.000 UL
LT0
2700 885 M
0 -21 V
1.000 UL
LT0
2617 877 M
83 -13 V
1.000 UL
LT0
2747 1117 M
33 -43 V
1.000 UL
LT0
2729 1094 M
51 -20 V
1.000 UL
LT0
2736 1002 M
12 -31 V
1.000 UL
LT0
2683 990 M
65 -19 V
1.000 UL
LT0
2698 907 M
2 -22 V
1.000 UL
LT0
2620 899 M
80 -14 V
1.000 UL
LT0
2729 1094 M
26 -40 V
1.000 UL
LT0
2700 1074 M
55 -20 V
1.000 UL
LT0
2695 932 M
3 -25 V
1.000 UL
LT0
2622 924 M
76 -17 V
1.000 UL
LT0
2719 1037 M
17 -35 V
1.000 UL
LT0
2673 1022 M
63 -20 V
1.000 UL
LT0
2603 824 M
-10 -13 V
1.000 UL
LT0
2496 821 M
97 -10 V
1.000 UL
LT0
2710 1162 M
37 -45 V
1.000 UL
LT0
2698 1136 M
49 -19 V
1.000 UL
LT0
2690 960 M
5 -28 V
1.000 UL
LT0
2622 950 M
73 -18 V
1.000 UL
LT0
2609 839 M
-6 -15 V
1.000 UL
LT0
2509 835 M
94 -11 V
1.000 UL
LT0
2698 1136 M
31 -42 V
1.000 UL
LT0
2676 1115 M
53 -21 V
1.000 UL
LT0
2700 1074 M
19 -37 V
1.000 UL
LT0
2660 1057 M
59 -20 V
1.000 UL
LT0
2683 990 M
7 -30 V
1.000 UL
LT0
2620 979 M
70 -19 V
1.000 UL
LT0
2614 857 M
-5 -18 V
1.000 UL
LT0
2518 851 M
91 -12 V
1.000 UL
LT0
2669 1211 M
41 -49 V
1.000 UL
LT0
2664 1182 M
46 -20 V
1.000 UL
LT0
2617 877 M
-3 -20 V
1.000 UL
LT0
2526 871 M
88 -14 V
1.000 UL
LT0
2673 1022 M
10 -32 V
1.000 UL
LT0
2616 1010 M
67 -20 V
1.000 UL
LT0
2676 1115 M
24 -41 V
1.000 UL
LT0
2643 1096 M
57 -22 V
1.000 UL
LT0
2664 1182 M
34 -46 V
1.000 UL
LT0
2648 1157 M
50 -21 V
1.000 UL
LT0
2620 899 M
-3 -22 V
1.000 UL
LT0
2532 892 M
85 -15 V
1.000 UL
LT0
2660 1057 M
13 -35 V
1.000 UL
LT0
2609 1044 M
64 -22 V
1.000 UL
LT0
2622 924 M
-2 -25 V
1.000 UL
LT0
2538 916 M
82 -17 V
1.000 UL
LT0
2648 1157 M
28 -42 V
1.000 UL
LT0
2622 1136 M
54 -21 V
1.000 UL
LT0
2624 1264 M
45 -53 V
1.000 UL
LT0
2625 1232 M
44 -21 V
1.000 UL
LT0
2622 950 M
0 -26 V
1.000 UL
LT0
2543 942 M
79 -18 V
1.000 UL
LT0
2625 1232 M
39 -50 V
1.000 UL
LT0
2616 1204 M
48 -22 V
1.000 UL
LT0
2643 1096 M
17 -39 V
1.000 UL
LT0
2599 1080 M
61 -23 V
1.000 UL
LT0
2620 979 M
2 -29 V
1.000 UL
LT0
2546 970 M
76 -20 V
1.000 UL
LT0
2616 1204 M
32 -47 V
1.000 UL
LT0
2597 1180 M
51 -23 V
1.000 UL
LT0
2622 1136 M
21 -40 V
1.000 UL
LT0
2584 1119 M
59 -23 V
1.000 UL
LT0
2616 1010 M
4 -31 V
1.000 UL
LT0
2547 1000 M
73 -21 V
1.000 UL
LT0
2509 835 M
-13 -14 V
1.000 UL
LT0
2396 832 M
100 -11 V
1.000 UL
LT0
2576 1318 M
48 -54 V
1.000 UL
LT0
2583 1284 M
41 -20 V
1.000 UL
LT0
2583 1284 M
42 -52 V
1.000 UL
LT0
2580 1254 M
45 -22 V
1.000 UL
LT0
2518 851 M
-9 -16 V
1.000 UL
LT0
2412 848 M
97 -13 V
1.000 UL
LT0
2609 1044 M
7 -34 V
1.000 UL
LT0
2547 1033 M
69 -23 V
1.000 UL
LT0
2597 1180 M
25 -44 V
1.000 UL
LT0
2566 1160 M
56 -24 V
1.000 UL
LT0
2580 1254 M
36 -50 V
1.000 UL
LT0
2568 1227 M
48 -23 V
1.000 UL
LT0
2526 871 M
-8 -20 V
1.000 UL
LT0
2424 866 M
94 -15 V
1.000 UL
LT0
2599 1080 M
10 -36 V
1.000 UL
LT0
2543 1068 M
66 -24 V
1.000 UL
LT0
2523 1376 M
53 -58 V
1.000 UL
LT0
2537 1338 M
39 -20 V
1.000 UL
LT0
2532 892 M
-6 -21 V
1.000 UL
LT0
2434 887 M
92 -16 V
1.000 UL
LT0
2537 1338 M
46 -54 V
1.000 UL
LT0
2540 1305 M
43 -21 V
1.000 UL
LT0
2584 1119 M
15 -39 V
1.000 UL
LT0
2535 1105 M
64 -25 V
1.000 UL
LT0
2568 1227 M
29 -47 V
1.000 UL
LT0
2544 1205 M
53 -25 V
1.000 UL
LT0
2538 916 M
-6 -24 V
1.000 UL
LT0
2444 910 M
88 -18 V
1.000 UL
LT0
2540 1305 M
40 -51 V
1.000 UL
LT0
2534 1276 M
46 -22 V
1.000 UL
LT0
2543 942 M
-5 -26 V
1.000 UL
LT0
2453 936 M
85 -20 V
1.000 UL
LT0
2566 1160 M
18 -41 V
1.000 UL
LT0
2524 1144 M
60 -25 V
1.000 UL
LT0
2487 1395 M
36 -19 V
1.000 UL
LT0
2487 1395 M
50 -57 V
1.000 UL
LT0
2497 1359 M
40 -21 V
1.000 UL
LT0
2546 970 M
-3 -28 V
1.000 UL
LT0
2461 963 M
82 -21 V
1.000 UL
LT0
2534 1276 M
34 -49 V
1.000 UL
LT0
2517 1251 M
51 -24 V
1.000 UL
LT0
2497 1359 M
43 -54 V
1.000 UL
LT0
2497 1328 M
43 -23 V
1.000 UL
LT0
2547 1000 M
-1 -30 V
1.000 UL
LT0
2468 993 M
78 -23 V
1.000 UL
LT0
2544 1205 M
22 -45 V
1.000 UL
LT0
2509 1186 M
57 -26 V
1.000 UL
LT0
2547 1033 M
0 -33 V
1.000 UL
LT0
2473 1024 M
74 -24 V
1.000 UL
LT0
2497 1328 M
37 -52 V
1.000 UL
LT0
2487 1300 M
47 -24 V
1.000 UL
LT0
2450 1415 M
37 -20 V
1.000 UL
LT0
2543 1068 M
4 -35 V
1.000 UL
LT0
2475 1058 M
72 -25 V
1.000 UL
LT0
2517 1251 M
27 -46 V
1.000 UL
LT0
2489 1230 M
55 -25 V
1.000 UL
LT0
2450 1415 M
47 -56 V
1.000 UL
LT0
2456 1381 M
41 -22 V
1.000 UL
LT0
2535 1105 M
8 -37 V
1.000 UL
LT0
2474 1094 M
69 -26 V
1.000 UL
LT0
2456 1381 M
41 -53 V
1.000 UL
LT0
2452 1351 M
45 -23 V
1.000 UL
LT0
2524 1144 M
11 -39 V
1.000 UL
LT0
2470 1131 M
65 -26 V
1.000 UL
LT0
2487 1300 M
30 -49 V
1.000 UL
LT0
2465 1277 M
52 -26 V
1.000 UL
LT0
2412 848 M
-16 -16 V
1.000 UL
LT0
2292 847 M
104 -15 V
1.000 UL
LT0
2413 1435 M
37 -20 V
1.000 UL
LT0
2509 1186 M
15 -42 V
1.000 UL
LT0
2462 1171 M
62 -27 V
1.000 UL
LT0
2424 866 M
-12 -18 V
1.000 UL
LT0
2311 863 M
101 -15 V
1.000 UL
LT0
2413 1435 M
43 -54 V
1.000 UL
LT0
2414 1403 M
42 -22 V
1.000 UL
LT0
2452 1351 M
35 -51 V
1.000 UL
LT0
2438 1325 M
49 -25 V
1.000 UL
LT0
2489 1230 M
20 -44 V
1.000 UL
LT0
2449 1214 M
60 -28 V
1.000 UL
LT0
2434 887 M
-10 -21 V
1.000 UL
LT0
2326 883 M
98 -17 V
1.000 UL
LT0
2374 1456 M
39 -21 V
1.000 UL
LT0
2414 1403 M
38 -52 V
1.000 UL
LT0
2406 1375 M
46 -24 V
1.000 UL
LT0
2444 910 M
-10 -23 V
1.000 UL
LT0
2340 906 M
94 -19 V
1.000 UL
LT0
2465 1277 M
24 -47 V
1.000 UL
LT0
2433 1258 M
56 -28 V
1.000 UL
LT0
2453 936 M
-9 -26 V
1.000 UL
LT0
2353 931 M
91 -21 V
1.000 UL
LT0
2374 1456 M
40 -53 V
1.000 UL
LT0
2372 1426 M
42 -23 V
1.000 UL
LT0
2438 1325 M
27 -48 V
1.000 UL
LT0
2412 1304 M
53 -27 V
1.000 UL
LT0
2461 963 M
-8 -27 V
1.000 UL
LT0
2365 958 M
88 -22 V
1.000 UL
LT0
2468 993 M
-7 -30 V
1.000 UL
LT0
2377 987 M
84 -24 V
1.000 UL
LT0
2334 1478 M
40 -22 V
1.000 UL
LT0
2473 1024 M
-5 -31 V
1.000 UL
LT0
2387 1018 M
81 -25 V
1.000 UL
LT0
2406 1375 M
32 -50 V
1.000 UL
LT0
2387 1352 M
51 -27 V
1.000 UL
LT0
2475 1058 M
-2 -34 V
1.000 UL
LT0
2395 1051 M
78 -27 V
1.000 UL
LT0
2474 1094 M
1 -36 V
1.000 UL
LT0
2401 1086 M
74 -28 V
1.000 UL
LT0
2470 1131 M
4 -37 V
1.000 UL
LT0
2404 1123 M
70 -29 V
1.000 UL
LT0
2372 1426 M
34 -51 V
1.000 UL
LT0
2359 1401 M
47 -26 V
1.000 UL
LT0
2462 1171 M
8 -40 V
1.000 UL
LT0
2403 1160 M
67 -29 V
1.000 UL
LT0
2334 1478 M
38 -52 V
1.000 UL
LT0
2449 1214 M
13 -43 V
1.000 UL
LT0
2327 1450 M
45 -24 V
1.000 UL
LT0
2397 1201 M
65 -30 V
1.000 UL
LT0
2294 1501 M
40 -23 V
1.000 UL
LT0
2433 1258 M
16 -44 V
1.000 UL
LT0
2388 1243 M
61 -29 V
1.000 UL
LT0
2412 1304 M
21 -46 V
1.000 UL
LT0
2374 1287 M
59 -29 V
1.000 UL
LT0
2387 1352 M
25 -48 V
1.000 UL
LT0
2356 1333 M
56 -29 V
1.000 UL
LT0
2359 1401 M
28 -49 V
1.000 UL
LT0
2335 1379 M
52 -27 V
1.000 UL
LT0
2327 1450 M
32 -49 V
1.000 UL
LT0
2310 1427 M
49 -26 V
1.000 UL
LT0
2294 1501 M
33 -51 V
1.000 UL
LT0
2282 1475 M
45 -25 V
1.000 UL
LT0
2252 1524 M
42 -23 V
1.000 UL
LT0
2311 863 M
-19 -16 V
1.000 UL
LT0
2184 864 M
108 -17 V
1.000 UL
LT0
2282 1475 M
-30 49 V
1.000 UL
LT0
2209 1548 M
43 -24 V
1.000 UL
LT0
2310 1427 M
-28 48 V
1.000 UL
LT0
2235 1501 M
47 -26 V
1.000 UL
LT0
2326 883 M
-15 -20 V
1.000 UL
LT0
2207 882 M
104 -19 V
1.000 UL
LT0
2335 1379 M
-25 48 V
1.000 UL
LT0
2260 1455 M
50 -28 V
1.000 UL
LT0
2356 1333 M
-21 46 V
1.000 UL
LT0
2281 1408 M
54 -29 V
1.000 UL
LT0
2374 1287 M
-18 46 V
1.000 UL
LT0
2299 1363 M
57 -30 V
1.000 UL
LT0
2388 1243 M
-14 44 V
1.000 UL
LT0
2314 1318 M
60 -31 V
1.000 UL
LT0
2397 1201 M
-9 42 V
1.000 UL
LT0
2324 1274 M
64 -31 V
1.000 UL
LT0
2403 1160 M
-6 41 V
1.000 UL
LT0
2331 1232 M
66 -31 V
1.000 UL
LT0
2404 1123 M
-1 37 V
1.000 UL
LT0
2332 1192 M
71 -32 V
1.000 UL
LT0
2401 1086 M
3 37 V
1.000 UL
LT0
2330 1153 M
74 -30 V
1.000 UL
LT0
2340 906 M
-14 -23 V
1.000 UL
LT0
2225 903 M
101 -20 V
1.000 UL
LT0
2395 1051 M
6 35 V
1.000 UL
LT0
2324 1117 M
77 -31 V
1.000 UL
LT0
2387 1018 M
8 33 V
1.000 UL
LT0
2315 1081 M
80 -30 V
1.000 UL
LT0
2353 931 M
-13 -25 V
1.000 UL
LT0
2242 928 M
98 -22 V
1.000 UL
LT0
2235 1501 M
-26 47 V
1.000 UL
LT0
2165 1573 M
44 -25 V
1.000 UL
LT0
2377 987 M
10 31 V
1.000 UL
LT0
2303 1047 M
84 -29 V
1.000 UL
LT0
2365 958 M
12 29 V
1.000 UL
LT0
2290 1014 M
87 -27 V
1.000 UL
LT0
2365 958 M
-12 -27 V
1.000 UL
LT0
2258 955 M
95 -24 V
1.000 UL
LT0
2274 984 M
91 -26 V
1.000 UL
LT0
2260 1455 M
-25 46 V
1.000 UL
LT0
2188 1528 M
47 -27 V
1.000 UL
LT0
2281 1408 M
-21 47 V
1.000 UL
LT0
2208 1483 M
52 -28 V
1.000 UL
LT0
2188 1528 M
-23 45 V
1.000 UL
LT0
2120 1599 M
45 -26 V
1.000 UL
LT0
2299 1363 M
-18 45 V
1.000 UL
LT0
2225 1439 M
56 -31 V
1.000 UL
LT0
2314 1318 M
-15 45 V
1.000 UL
LT0
2240 1394 M
59 -31 V
1.000 UL
LT0
2208 1483 M
-20 45 V
1.000 UL
LT0
2138 1556 M
50 -28 V
1.000 UL
LT0
2324 1274 M
-10 44 V
1.000 UL
LT0
2251 1351 M
63 -33 V
1.000 UL
LT0
2331 1232 M
-7 42 V
1.000 UL
LT0
2258 1308 M
66 -34 V
1.000 UL
LT0
2138 1556 M
-18 43 V
1.000 UL
LT0
2074 1625 M
46 -26 V
1.000 UL
LT0
2225 1439 M
-17 44 V
1.000 UL
LT0
2154 1513 M
54 -30 V
1.000 UL
LT0
2332 1192 M
-1 40 V
1.000 UL
LT0
2261 1266 M
70 -34 V
1.000 UL
LT0
2330 1153 M
2 39 V
1.000 UL
LT0
2260 1226 M
72 -34 V
1.000 UL
LT0
2240 1394 M
-15 45 V
1.000 UL
LT0
2168 1470 M
57 -31 V
1.000 UL
LT0
2154 1513 M
-16 43 V
1.000 UL
LT0
2087 1585 M
51 -29 V
1.000 UL
LT0
2087 1585 M
-13 40 V
1.000 UL
LT0
2027 1653 M
47 -28 V
1.000 UL
LT0
2324 1117 M
6 36 V
1.000 UL
LT0
2254 1187 M
76 -34 V
1.000 UL
LT0
2251 1351 M
-11 43 V
1.000 UL
LT0
2179 1427 M
61 -33 V
1.000 UL
LT0
2315 1081 M
9 36 V
1.000 UL
LT0
2245 1149 M
79 -32 V
1.000 UL
LT0
2168 1470 M
-14 43 V
1.000 UL
LT0
2099 1544 M
55 -31 V
1.000 UL
LT0
2035 1615 M
-8 38 V
1.000 UL
LT0
1978 1681 M
49 -28 V
1.000 UL
LT0
2258 1308 M
-7 43 V
1.000 UL
LT0
2186 1385 M
65 -34 V
1.000 UL
LT0
2099 1544 M
-12 41 V
1.000 UL
LT0
2035 1615 M
52 -30 V
1.000 UL
LT0
2303 1047 M
12 34 V
1.000 UL
LT0
2232 1114 M
83 -33 V
1.000 UL
LT0
2207 882 M
-23 -18 V
1.000 UL
LT0
2072 885 M
112 -21 V
1.000 UL
LT0
2179 1427 M
-11 43 V
1.000 UL
LT0
2108 1503 M
60 -33 V
1.000 UL
LT0
2290 1014 M
13 33 V
1.000 UL
LT0
2216 1079 M
87 -32 V
1.000 UL
LT0
2261 1266 M
-3 42 V
1.000 UL
LT0
2189 1344 M
69 -36 V
1.000 UL
LT0
1981 1646 M
-3 35 V
1.000 UL
LT0
1928 1710 M
50 -29 V
1.000 UL
LT0
2274 984 M
16 30 V
1.000 UL
LT0
2199 1045 M
91 -31 V
1.000 UL
LT0
2225 903 M
-18 -21 V
1.000 UL
LT0
2097 904 M
110 -22 V
1.000 UL
LT0
2108 1503 M
-9 41 V
1.000 UL
LT0
2042 1577 M
57 -33 V
1.000 UL
LT0
2042 1577 M
-7 38 V
1.000 UL
LT0
1981 1646 M
54 -31 V
1.000 UL
LT0
2260 1226 M
1 40 V
1.000 UL
LT0
2189 1303 M
72 -37 V
1.000 UL
LT0
2258 955 M
16 29 V
1.000 UL
LT0
2180 1013 M
94 -29 V
1.000 UL
LT0
2186 1385 M
-7 42 V
1.000 UL
LT0
2115 1463 M
64 -36 V
1.000 UL
LT0
2242 928 M
-17 -25 V
1.000 UL
LT0
2119 927 M
106 -24 V
1.000 UL
LT0
1926 1678 M
2 32 V
1.000 UL
LT0
1877 1740 M
51 -30 V
1.000 UL
LT0
2242 928 M
16 27 V
1.000 UL
LT0
2160 982 M
98 -27 V
1.000 UL
LT0
2139 953 M
103 -25 V
1.000 UL
LT0
2254 1187 M
6 39 V
1.000 UL
LT0
2184 1263 M
76 -37 V
1.000 UL
LT0
1983 1611 M
-2 35 V
1.000 UL
LT0
1926 1678 M
55 -32 V
1.000 UL
LT0
2115 1463 M
-7 40 V
1.000 UL
LT0
2047 1538 M
61 -35 V
1.000 UL
LT0
1868 1712 M
9 28 V
1.000 UL
LT0
1824 1771 M
53 -31 V
1.000 UL
LT0
2189 1344 M
-3 41 V
1.000 UL
LT0
2118 1422 M
68 -37 V
1.000 UL
LT0
2047 1538 M
-5 39 V
1.000 UL
LT0
1983 1611 M
59 -34 V
1.000 UL
LT0
2245 1149 M
9 38 V
1.000 UL
LT0
2175 1224 M
79 -37 V
1.000 UL
LT0
1809 1747 M
15 24 V
1.000 UL
LT0
1770 1803 M
54 -32 V
1.000 UL
LT0
1922 1646 M
4 32 V
1.000 UL
LT0
1868 1712 M
58 -34 V
1.000 UL
LT0
2189 1303 M
0 41 V
1.000 UL
LT0
2118 1381 M
71 -37 V
1.000 UL
LT0
2118 1422 M
-3 41 V
1.000 UL
LT0
2049 1499 M
66 -36 V
1.000 UL
LT0
1749 1782 M
21 21 V
1.000 UL
LT0
1715 1837 M
55 -34 V
1.000 UL
LT0
2232 1114 M
13 35 V
1.000 UL
LT0
2162 1186 M
83 -37 V
1.000 UL
LT0
1983 1575 M
0 36 V
1.000 UL
LT0
1922 1646 M
61 -35 V
1.000 UL
LT0
2049 1499 M
-2 39 V
1.000 UL
LT0
1983 1575 M
64 -37 V
1.000 UL
LT0
1686 1820 M
29 17 V
1.000 UL
LT0
1657 1871 M
58 -34 V
1.000 UL
LT0
1859 1683 M
9 29 V
1.000 UL
LT0
1809 1747 M
59 -35 V
1.000 UL
LT0
2184 1263 M
5 40 V
1.000 UL
LT0
2113 1342 M
76 -39 V
1.000 UL
LT0
1621 1858 M
36 13 V
1.000 UL
LT0
2216 1079 M
16 35 V
1.000 UL
LT0
2145 1149 M
87 -35 V
1.000 UL
LT0
2118 1381 M
0 41 V
1.000 UL
LT0
2048 1461 M
70 -39 V
1.000 UL
LT0
1794 1721 M
15 26 V
1.000 UL
LT0
1749 1782 M
60 -35 V
1.000 UL
LT0
1916 1613 M
6 33 V
1.000 UL
LT0
1859 1683 M
63 -37 V
1.000 UL
LT0
2048 1461 M
1 38 V
1.000 UL
LT0
1980 1538 M
69 -39 V
1.000 UL
LT0
2199 1045 M
17 34 V
1.000 UL
LT0
2126 1114 M
90 -35 V
1.000 UL
LT0
2175 1224 M
9 39 V
1.000 UL
LT0
2105 1302 M
79 -39 V
1.000 UL
LT0
1980 1538 M
3 37 V
1.000 UL
LT0
1916 1613 M
67 -38 V
1.000 UL
LT0
1727 1761 M
22 21 V
1.000 UL
LT0
1686 1820 M
63 -38 V
1.000 UL
LT0
2113 1342 M
5 39 V
1.000 UL
LT0
2043 1422 M
75 -41 V
1.000 UL
LT0
1847 1653 M
12 30 V
1.000 UL
LT0
1794 1721 M
65 -38 V
1.000 UL
LT0
2180 1013 M
19 32 V
1.000 UL
LT0
2104 1079 M
95 -34 V
1.000 UL
LT0
1657 1802 M
29 18 V
1.000 UL
LT0
1621 1858 M
65 -38 V
1.000 UL
LT0
2162 1186 M
13 38 V
1.000 UL
LT0
2092 1264 M
83 -40 V
1.000 UL
LT0
2097 904 M
-25 -19 V
1.000 UL
LT0
1954 909 M
118 -24 V
1.000 UL
LT0
2043 1422 M
5 39 V
1.000 UL
LT0
1974 1501 M
74 -40 V
1.000 UL
LT0
1908 1579 M
8 34 V
1.000 UL
LT0
1847 1653 M
69 -40 V
1.000 UL
LT0
1584 1845 M
37 13 V
1.000 UL
LT0
2160 982 M
20 31 V
1.000 UL
LT0
2081 1045 M
99 -32 V
1.000 UL
LT0
1777 1694 M
17 27 V
1.000 UL
LT0
1727 1761 M
67 -40 V
1.000 UL
LT0
1974 1501 M
6 37 V
1.000 UL
LT0
1908 1579 M
72 -41 V
1.000 UL
LT0
2105 1302 M
8 40 V
1.000 UL
LT0
2034 1383 M
79 -41 V
1.000 UL
LT0
2119 927 M
-22 -23 V
1.000 UL
LT0
1983 929 M
114 -25 V
1.000 UL
LT0
2139 953 M
21 29 V
1.000 UL
LT0
2057 1013 M
103 -31 V
1.000 UL
LT0
2119 927 M
20 26 V
1.000 UL
LT0
2032 983 M
107 -30 V
1.000 UL
LT0
2008 955 M
111 -28 V
1.000 UL
LT0
2145 1149 M
17 37 V
1.000 UL
LT0
2075 1226 M
87 -40 V
1.000 UL
LT0
1702 1738 M
25 23 V
1.000 UL
LT0
1657 1802 M
70 -41 V
1.000 UL
LT0
1834 1622 M
13 31 V
1.000 UL
LT0
1777 1694 M
70 -41 V
1.000 UL
LT0
2034 1383 M
9 39 V
1.000 UL
LT0
1965 1465 M
78 -43 V
1.000 UL
LT0
1625 1784 M
32 18 V
1.000 UL
LT0
1584 1845 M
73 -43 V
1.000 UL
LT0
2092 1264 M
13 38 V
1.000 UL
LT0
2022 1345 M
83 -43 V
1.000 UL
LT0
1897 1545 M
11 34 V
1.000 UL
LT0
1834 1622 M
74 -43 V
1.000 UL
LT0
1965 1465 M
9 36 V
1.000 UL
LT0
1897 1545 M
77 -44 V
1.000 UL
LT0
2126 1114 M
19 35 V
1.000 UL
LT0
2054 1189 M
91 -40 V
1.000 UL
LT0
1544 1831 M
40 14 V
1.000 UL
LT0
1757 1667 M
20 27 V
1.000 UL
LT0
1702 1738 M
75 -44 V
1.000 UL
LT0
2022 1345 M
12 38 V
1.000 UL
LT0
1952 1428 M
82 -45 V
1.000 UL
LT0
2075 1226 M
17 38 V
1.000 UL
LT0
2005 1307 M
87 -43 V
1.000 UL
LT0
2104 1079 M
22 35 V
1.000 UL
LT0
2031 1152 M
95 -38 V
1.000 UL
LT0
1817 1590 M
17 32 V
1.000 UL
LT0
1757 1667 M
77 -45 V
1.000 UL
LT0
1676 1714 M
26 24 V
1.000 UL
LT0
1625 1784 M
77 -46 V
1.000 UL
LT0
1952 1428 M
13 37 V
1.000 UL
LT0
1883 1510 M
82 -45 V
1.000 UL
LT0
1883 1510 M
14 35 V
1.000 UL
LT0
1817 1590 M
80 -45 V
1.000 UL
LT0
1591 1764 M
34 20 V
1.000 UL
LT0
1544 1831 M
81 -47 V
1.000 UL
LT0
2081 1045 M
23 34 V
1.000 UL
LT0
2005 1117 M
99 -38 V
1.000 UL
LT0
1734 1639 M
23 28 V
1.000 UL
LT0
1676 1714 M
81 -47 V
1.000 UL
LT0
2054 1189 M
21 37 V
1.000 UL
LT0
1984 1270 M
91 -44 V
1.000 UL
LT0
2005 1307 M
17 38 V
1.000 UL
LT0
1935 1391 M
87 -46 V
1.000 UL
LT0
1503 1817 M
41 14 V
1.000 UL
LT0
2057 1013 M
24 32 V
1.000 UL
LT0
1977 1082 M
104 -37 V
1.000 UL
LT0
1799 1559 M
18 31 V
1.000 UL
LT0
1734 1639 M
83 -49 V
1.000 UL
LT0
1935 1391 M
17 37 V
1.000 UL
LT0
1866 1475 M
86 -47 V
1.000 UL
LT0
1647 1690 M
29 24 V
1.000 UL
LT0
1591 1764 M
85 -50 V
1.000 UL
LT0
1866 1475 M
17 35 V
1.000 UL
LT0
1799 1559 M
84 -49 V
1.000 UL
LT0
1983 929 M
-29 -20 V
1.000 UL
LT0
1831 937 M
123 -28 V
1.000 UL
LT0
2032 983 M
25 30 V
1.000 UL
LT0
1949 1049 M
108 -36 V
1.000 UL
LT0
2031 1152 M
23 37 V
1.000 UL
LT0
1959 1232 M
95 -43 V
1.000 UL
LT0
1984 1270 M
21 37 V
1.000 UL
LT0
1914 1354 M
91 -47 V
1.000 UL
LT0
1555 1744 M
36 20 V
1.000 UL
LT0
1503 1817 M
88 -53 V
1.000 UL
LT0
2008 955 M
-25 -26 V
1.000 UL
LT0
2008 955 M
24 28 V
1.000 UL
LT0
1863 959 M
120 -30 V
1.000 UL
LT0
1920 1016 M
112 -33 V
1.000 UL
LT0
1709 1610 M
25 29 V
1.000 UL
LT0
1647 1690 M
87 -51 V
1.000 UL
LT0
1891 986 M
117 -31 V
1.000 UL
LT0
1459 1801 M
44 16 V
1.000 UL
LT0
1914 1354 M
21 37 V
1.000 UL
LT0
1844 1440 M
91 -49 V
1.000 UL
LT0
1776 1526 M
23 33 V
1.000 UL
LT0
1709 1610 M
90 -51 V
1.000 UL
LT0
2005 1117 M
26 35 V
1.000 UL
LT0
1932 1195 M
99 -43 V
1.000 UL
LT0
1844 1440 M
22 35 V
1.000 UL
LT0
1776 1526 M
90 -51 V
1.000 UL
LT0
1615 1664 M
32 26 V
1.000 UL
LT0
1555 1744 M
92 -54 V
1.000 UL
LT0
1959 1232 M
25 38 V
1.000 UL
LT0
1889 1317 M
95 -47 V
1.000 UL
LT0
1977 1082 M
28 35 V
1.000 UL
LT0
1901 1159 M
104 -42 V
1.000 UL
LT0
1516 1722 M
39 22 V
1.000 UL
LT0
1459 1801 M
96 -57 V
1.000 UL
LT0
1680 1580 M
29 30 V
1.000 UL
LT0
1615 1664 M
94 -54 V
1.000 UL
LT0
1889 1317 M
25 37 V
1.000 UL
LT0
1818 1405 M
96 -51 V
1.000 UL
LT0
1412 1784 M
47 17 V
1.000 UL
LT0
1749 1493 M
27 33 V
1.000 UL
LT0
1680 1580 M
96 -54 V
1.000 UL
LT0
1818 1405 M
26 35 V
1.000 UL
LT0
1749 1493 M
95 -53 V
1.000 UL
LT0
1932 1195 M
27 37 V
1.000 UL
LT0
1860 1280 M
99 -48 V
1.000 UL
LT0
1949 1049 M
28 33 V
1.000 UL
LT0
1869 1124 M
108 -42 V
1.000 UL
LT0
1580 1638 M
35 26 V
1.000 UL
LT0
1516 1722 M
99 -58 V
1.000 UL
LT0
1920 1016 M
29 33 V
1.000 UL
LT0
1835 1089 M
114 -40 V
1.000 UL
LT0
1860 1280 M
29 37 V
1.000 UL
LT0
1789 1369 M
100 -52 V
1.000 UL
LT0
1648 1550 M
32 30 V
1.000 UL
LT0
1580 1638 M
100 -58 V
1.000 UL
LT0
1474 1700 M
42 22 V
1.000 UL
LT0
1412 1784 M
104 -62 V
1.000 UL
LT0
1901 1159 M
31 36 V
1.000 UL
LT0
1827 1243 M
105 -48 V
1.000 UL
LT0
1863 959 M
-32 -22 V
1.000 UL
LT0
1703 969 M
128 -32 V
1.000 UL
LT0
1891 986 M
29 30 V
1.000 UL
LT0
1802 1055 M
118 -39 V
1.000 UL
LT0
1789 1369 M
29 36 V
1.000 UL
LT0
1718 1459 M
100 -54 V
1.000 UL
LT0
1718 1459 M
31 34 V
1.000 UL
LT0
1648 1550 M
101 -57 V
1.000 UL
LT0
1891 986 M
-28 -27 V
1.000 UL
LT0
1737 993 M
126 -34 V
1.000 UL
LT0
1362 1765 M
50 19 V
1.000 UL
LT0
1770 1022 M
121 -36 V
1.000 UL
LT0
1541 1610 M
39 28 V
1.000 UL
LT0
1474 1700 M
106 -62 V
1.000 UL
LT0
1869 1124 M
32 35 V
1.000 UL
LT0
1793 1206 M
108 -47 V
1.000 UL
LT0
1827 1243 M
33 37 V
1.000 UL
LT0
1755 1333 M
105 -53 V
1.000 UL
LT0
1611 1518 M
37 32 V
1.000 UL
LT0
1541 1610 M
107 -60 V
1.000 UL
LT0
1428 1676 M
46 24 V
1.000 UL
LT0
1362 1765 M
112 -65 V
1.000 UL
LT0
1755 1333 M
34 36 V
1.000 UL
LT0
1683 1425 M
106 -56 V
1.000 UL
LT0
1683 1425 M
35 34 V
1.000 UL
LT0
1611 1518 M
107 -59 V
1.000 UL
LT0
1835 1089 M
34 35 V
1.000 UL
LT0
1755 1169 M
114 -45 V
1.000 UL
LT0
1309 1745 M
53 20 V
1.000 UL
LT0
1793 1206 M
34 37 V
1.000 UL
LT0
1718 1296 M
109 -53 V
1.000 UL
LT0
1498 1582 M
43 28 V
1.000 UL
LT0
1428 1676 M
113 -66 V
1.000 UL
LT0
1802 1055 M
33 34 V
1.000 UL
LT0
1717 1133 M
118 -44 V
1.000 UL
LT0
1718 1296 M
37 37 V
1.000 UL
LT0
1644 1390 M
111 -57 V
1.000 UL
LT0
1571 1486 M
40 32 V
1.000 UL
LT0
1498 1582 M
113 -64 V
1.000 UL
LT0
1644 1390 M
39 35 V
1.000 UL
LT0
1571 1486 M
112 -61 V
1.000 UL
LT0
1379 1650 M
49 26 V
1.000 UL
LT0
1309 1745 M
119 -69 V
1.000 UL
LT0
1737 993 M
-34 -24 V
1.000 UL
LT0
1566 1006 M
137 -37 V
1.000 UL
LT0
1770 1022 M
32 33 V
1.000 UL
LT0
1678 1098 M
124 -43 V
1.000 UL
LT0
1755 1169 M
38 37 V
1.000 UL
LT0
1677 1259 M
116 -53 V
1.000 UL
LT0
1737 993 M
33 29 V
1.000 UL
LT0
1640 1064 M
130 -42 V
1.000 UL
LT0
1604 1033 M
133 -40 V
1.000 UL
LT0
1252 1724 M
57 21 V
1.000 UL
LT0
1452 1552 M
46 30 V
1.000 UL
LT0
1379 1650 M
119 -68 V
1.000 UL
LT0
1677 1259 M
41 37 V
1.000 UL
LT0
1601 1354 M
117 -58 V
1.000 UL
LT0
1717 1133 M
38 36 V
1.000 UL
LT0
1635 1221 M
120 -52 V
1.000 UL
LT0
1526 1452 M
45 34 V
1.000 UL
LT0
1452 1552 M
119 -66 V
1.000 UL
LT0
1601 1354 M
43 36 V
1.000 UL
LT0
1526 1452 M
118 -62 V
1.000 UL
LT0
1325 1623 M
54 27 V
1.000 UL
LT0
1252 1724 M
127 -74 V
1.000 UL
LT0
1678 1098 M
39 35 V
1.000 UL
LT0
1591 1184 M
126 -51 V
1.000 UL
LT0
1191 1700 M
61 24 V
1.000 UL
LT0
1635 1221 M
42 38 V
1.000 UL
LT0
1555 1317 M
122 -58 V
1.000 UL
LT0
1401 1520 M
51 32 V
1.000 UL
LT0
1325 1623 M
127 -71 V
1.000 UL
LT0
1555 1317 M
46 37 V
1.000 UL
LT0
1478 1417 M
123 -63 V
1.000 UL
LT0
1640 1064 M
38 34 V
1.000 UL
LT0
1546 1146 M
132 -48 V
1.000 UL
LT0
1478 1417 M
48 35 V
1.000 UL
LT0
1401 1520 M
125 -68 V
1.000 UL
LT0
1604 1033 M
-38 -27 V
1.000 UL
LT0
1422 1048 M
144 -42 V
1.000 UL
LT0
1604 1033 M
36 31 V
1.000 UL
LT0
1503 1111 M
137 -47 V
1.000 UL
LT0
1268 1594 M
57 29 V
1.000 UL
LT0
1191 1700 M
134 -77 V
1.000 UL
LT0
1462 1077 M
142 -44 V
1.000 UL
LT0
1591 1184 M
44 37 V
1.000 UL
LT0
1507 1279 M
128 -58 V
1.000 UL
LT0
1125 1675 M
66 25 V
1.000 UL
LT0
1346 1487 M
55 33 V
1.000 UL
LT0
1268 1594 M
133 -74 V
1.000 UL
LT0
1507 1279 M
48 38 V
1.000 UL
LT0
1426 1381 M
129 -64 V
1.000 UL
LT0
1426 1381 M
52 36 V
1.000 UL
LT0
1346 1487 M
132 -70 V
1.000 UL
LT0
1546 1146 M
45 38 V
1.000 UL
LT0
1457 1241 M
134 -57 V
1.000 UL
LT0
1206 1563 M
62 31 V
1.000 UL
LT0
1125 1675 M
143 -81 V
1.000 UL
LT0
1503 1111 M
43 35 V
1.000 UL
LT0
1406 1202 M
140 -56 V
1.000 UL
LT0
1457 1241 M
50 38 V
1.000 UL
LT0
1371 1343 M
136 -64 V
1.000 UL
LT0
1462 1077 M
-40 -29 V
1.000 UL
LT0
1268 1097 M
154 -49 V
1.000 UL
LT0
1287 1452 M
59 35 V
1.000 UL
LT0
1206 1563 M
140 -76 V
1.000 UL
LT0
1056 1647 M
69 28 V
1.000 UL
LT0
1371 1343 M
55 38 V
1.000 UL
LT0
1287 1452 M
139 -71 V
1.000 UL
LT0
1462 1077 M
41 34 V
1.000 UL
LT0
1357 1164 M
146 -53 V
1.000 UL
LT0
1311 1129 M
151 -52 V
1.000 UL
LT0
1406 1202 M
51 39 V
1.000 UL
LT0
1314 1305 M
143 -64 V
1.000 UL
LT0
1140 1530 M
66 33 V
1.000 UL
LT0
1056 1647 M
150 -84 V
1.000 UL
LT0
1226 1415 M
61 37 V
1.000 UL
LT0
1140 1530 M
147 -78 V
1.000 UL
LT0
1314 1305 M
57 38 V
1.000 UL
LT0
1226 1415 M
145 -72 V
1.000 UL
LT0
981 1616 M
75 31 V
1.000 UL
LT0
1357 1164 M
49 38 V
1.000 UL
LT0
1257 1265 M
149 -63 V
1.000 UL
LT0
1311 1129 M
-43 -32 V
1.000 UL
LT0
1104 1151 M
164 -54 V
1.000 UL
LT0
1311 1129 M
46 35 V
1.000 UL
LT0
1201 1225 M
156 -61 V
1.000 UL
LT0
1070 1494 M
70 36 V
1.000 UL
LT0
981 1616 M
159 -86 V
1.000 UL
LT0
1150 1186 M
161 -57 V
1.000 UL
LT0
1257 1265 M
57 40 V
1.000 UL
LT0
1161 1376 M
153 -71 V
1.000 UL
LT0
1161 1376 M
65 39 V
1.000 UL
LT0
1070 1494 M
156 -79 V
1.000 UL
LT0
903 1582 M
78 34 V
1.000 UL
LT0
1201 1225 M
56 40 V
1.000 UL
LT0
1097 1336 M
160 -71 V
1.000 UL
LT0
1150 1186 M
-46 -35 V
1.000 UL
LT0
928 1213 M
176 -62 V
1.000 UL
LT0
998 1456 M
72 38 V
1.000 UL
LT0
903 1582 M
167 -88 V
1.000 UL
LT0
1097 1336 M
64 40 V
1.000 UL
LT0
998 1456 M
163 -80 V
1.000 UL
LT0
1150 1186 M
51 39 V
1.000 UL
LT0
1034 1294 M
167 -69 V
1.000 UL
LT0
977 1253 M
173 -67 V
1.000 UL
LT0
822 1545 M
81 37 V
1.000 UL
LT0
1034 1294 M
63 42 V
1.000 UL
LT0
925 1415 M
172 -79 V
1.000 UL
LT0
925 1415 M
73 41 V
1.000 UL
LT0
822 1545 M
176 -89 V
1.000 UL
LT0
977 1253 M
-49 -40 V
1.000 UL
LT0
739 1284 M
189 -71 V
1.000 UL
LT0
977 1253 M
57 41 V
1.000 UL
LT0
854 1372 M
180 -78 V
1.000 UL
LT0
790 1328 M
187 -75 V
1.000 UL
LT0
740 1504 M
82 41 V
1.000 UL
LT0
854 1372 M
71 43 V
1.000 UL
LT0
740 1504 M
185 -89 V
1.000 UL
LT0
790 1328 M
-51 -44 V
1.000 UL
LT0
536 1364 M
203 -80 V
1.000 UL
LT0
790 1328 M
64 44 V
1.000 UL
LT0
660 1461 M
194 -89 V
1.000 UL
LT0
660 1461 M
80 43 V
1.000 UL
LT0
588 1413 M
202 -85 V
1.000 UL
LT0
588 1413 M
-52 -49 V
1.000 UL
LT0
588 1413 M
72 48 V
1.000 UL
LT0
1.000 UL
LTb
1685 281 M
3117 721 L
1.000 UL
LTb
1685 281 M
483 806 L
1.000 UL
LTb
483 806 M
865 265 V
1.000 UL
LTb
3117 721 M
-164 72 V
1.000 UL
LTb
483 1539 M
0 -733 V
1.000 UL
LTa
1685 281 M
483 806 L
1.000 UL
LTb
1685 281 M
-75 33 V
1.000 UL
LTb
1.000 UL
LTb
1.000 UL
LTb
559 773 M
-76 33 V
1.000 UL
LTb
1828 325 M
-37 16 V
1.000 UL
LTb
1.000 UL
LTb
664 833 M
-38 17 V
1.000 UL
LTa
1971 369 M
770 894 L
1.000 UL
LTb
1971 369 M
-76 33 V
1.000 UL
LTb
1.000 UL
LTb
1.000 UL
LTb
845 861 M
-75 33 V
1.000 UL
LTb
2114 413 M
-38 17 V
1.000 UL
LTb
1.000 UL
LTb
951 921 M
-38 17 V
1.000 UL
LTa
2257 457 M
1056 982 L
1.000 UL
LTb
2257 457 M
-75 33 V
1.000 UL
LTb
1.000 UL
LTb
1.000 UL
LTb
1132 949 M
-76 33 V
1.000 UL
LTb
2401 501 M
-38 17 V
1.000 UL
LTb
1.000 UL
LTb
1237 1009 M
-38 17 V
1.000 UL
LTa
2544 545 M
1343 1070 L
1.000 UL
LTb
2544 545 M
-76 33 V
1.000 UL
LTb
1.000 UL
LTb
1.000 UL
LTb
1418 1037 M
-75 33 V
1.000 UL
LTb
2687 589 M
-38 17 V
1.000 UL
LTb
1.000 UL
LTa
2830 633 M
2363 837 L
1.000 UL
LTb
2830 633 M
-75 33 V
1.000 UL
LTb
1.000 UL
LTb
1.000 UL
LTb
2974 677 M
-38 17 V
1.000 UL
LTb
1.000 UL
LTa
3117 721 M
-164 72 V
1.000 UL
LTb
3117 721 M
-76 33 V
1.000 UL
LTb
1.000 UL
LTb
LTb
1.000 UL
LTa
1685 281 M
3117 721 L
1.000 UL
LTb
1685 281 M
49 15 V
1.000 UL
LTb
1.000 UL
LTb
3068 706 M
49 15 V
1.000 UL
LTb
1565 333 M
24 8 V
1.000 UL
LTb
2972 766 M
25 8 V
1.000 UL
LTa
1445 386 M
2785 798 L
1.000 UL
LTb
1445 386 M
48 15 V
1.000 UL
LTb
1.000 UL
LTb
1325 438 M
24 8 V
1.000 UL
LTa
1204 491 M
2341 840 L
1.000 UL
LTb
1204 491 M
49 15 V
1.000 UL
LTb
1.000 UL
LTb
1084 543 M
24 8 V
1.000 UL
LTa
964 596 M
1971 905 L
1.000 UL
LTb
964 596 M
48 15 V
1.000 UL
LTb
1.000 UL
LTb
844 648 M
24 8 V
1.000 UL
LTa
724 701 M
923 283 V
1.000 UL
LTb
724 701 M
48 14 V
1.000 UL
LTb
1.000 UL
LTb
603 753 M
25 8 V
1.000 UL
LTa
483 806 M
865 265 V
1.000 UL
LTb
483 806 M
49 14 V
1.000 UL
LTb
LTb
1.000 UL
LTb
514 806 M
-31 0 V
1.000 UL
LTb
546 910 M
-63 0 V
1.000 UL
LTb
1.000 UL
LTb
514 1015 M
-31 0 V
1.000 UL
LTb
546 1120 M
-63 0 V
1.000 UL
LTb
1.000 UL
LTb
514 1224 M
-31 0 V
1.000 UL
LTb
546 1329 M
-63 0 V
1.000 UL
LTb
1.000 UL
LTb
514 1434 M
-31 0 V
1.000 UL
LTb
546 1539 M
-63 0 V
1.000 UL
LTb
LTb
1.000 UP
stroke
grestore
end
showpage
}}%
\put(482,1722){\makebox(0,0){$D_{\rho,\tilde{\rho}}(R,D_{\rho})$}}%
\put(357,1539){\makebox(0,0)[r]{ 1}}%
\put(357,1329){\makebox(0,0)[r]{ 0.8}}%
\put(357,1120){\makebox(0,0)[r]{ 0.6}}%
\put(357,910){\makebox(0,0)[r]{ 0.4}}%
\put(726,433){\makebox(0,0){$D_{\rho}$}}%
\put(445,782){\makebox(0,0){ 1}}%
\put(685,677){\makebox(0,0){ 0.8}}%
\put(926,572){\makebox(0,0){ 0.6}}%
\put(1166,467){\makebox(0,0){ 0.4}}%
\put(1407,362){\makebox(0,0){ 0.2}}%
\put(1647,257){\makebox(0,0){ 0}}%
\put(2701,370){\makebox(0,0){$R$}}%
\put(3177,669){\makebox(0,0)[l]{ 1}}%
\put(2890,581){\makebox(0,0)[l]{ 0.8}}%
\put(2604,493){\makebox(0,0)[l]{ 0.6}}%
\put(2317,405){\makebox(0,0)[l]{ 0.4}}%
\put(2031,317){\makebox(0,0)[l]{ 0.2}}%
\end{picture}%
\endgroup
\endinput

